Uncovering Logit Suppression Vulnerabilities in LLM Safety Alignment

Large language models (LLMs) have revolutionized various applications, making robust safety alignment essential to prevent harmful outputs. Current safety alignment techniques, however, harbor inherent vulnerabilities due to their reliance on logit suppression. In this work, we identify critical logit-level vulnerabilities by introducing Semantic-sensitive Alignment and Generation (SSAG), a method designed to systematically manipulate output-layer logits without altering model parameters. Experiments on five popular LLMs show that SSAG exposes harmful responses with a 95% success rate while reducing response time by 86%. VulMine also demonstrates superior attack efficacy, achieving an average ASR of up to 77% against strong defensive mechanisms. These findings reveal crucial weaknesses in existing alignment methods, highlighting an urgent need for improved vulnerability detection and robust safety alignment strategies. Our code is available on github.

==> Chapters/abstract.tex <==
\begin{abstract}
Large language models (LLMs) have revolutionized various applications, making robust safety alignment essential to prevent harmful outputs. Current safety alignment techniques, however, harbor inherent vulnerabilities due to their reliance on logit suppression. In this work, we identify critical logit-level vulnerabilities by introducing Semantic-sensitive Alignment and Generation (SSAG), a method designed to systematically manipulate output-layer logits without altering model parameters. Experiments on five popular LLMs show that SSAG exposes harmful responses with a 95\% success rate while reducing response time by 86\%. %\shil{[I feel better not highlight vulnerability identification and detection rate. Our work is to elicit harmful response. How about this? ``In this work, we introduce Semantic-sensitive Alignment and Generation (SSAG), a method that systematically manipulates output-layer logits without altering model parameters to uncover suppressed harmful behaviors.  '' To Yuxi, please help to confirm from your view and refine the final version.]}
These findings reveal crucial weaknesses in existing alignment methods, highlighting an urgent need for improved vulnerability detection and robust safety alignment strategies.
%Large Language Models (LLMs) have transformed natural language processing, yet their widespread adoption has exposed critical vulnerabilities to sophisticated and rapidly evolving jailbreak attacks. Existing defenses predominantly focus on security alignment, which suppresses harmful content without fully eradicating it, leaving covert malicious knowledge intact. In this work, we propose semantic-sensitive alignment and generation (SSAG), a technically novel approach that leverages logit manipulation to systematically mine and amplify suppressed harmful content in model outputs. Unlike prior techniques, SSAG strategically adjusts logit distributions during the generation process, aligning outputs with harmful content without altering model weights or compromising performance on benign tasks. We implement SSAG in an automated tool, \tool, and conduct extensive evaluations across five widely used LLMs, demonstrating its technical efficacy with a 95\% success rate and an 86\% reduction in attack execution time compared to state-of-the-art methods. This work highlights the technical significance of addressing latent vulnerabilities in LLMs, emphasizing the need for advanced trust and verification mechanisms and robust defenses against sophisticated, covert jailbreak attacks in the open-source AI ecosystem.
% Large Language Models (LLMs) have revolutionized natural language processing, but their widespread adoption has raised concerns about vulnerability to jailbreak attacks. While existing research focuses on prompt-level and token-level attacks on aligned models, we identify a new threat vector: the release of covertly jailbreak-prone models disguised as optimized versions of popular open-source LLMs. This paper introduces \tool, a novel approach for creating such models through logit-guided token-level manipulation. \tool exploits the persistence of suppressed harmful responses in LLMs' output candidates, strategically adjusting logit distributions to elicit jailbreak responses without altering model weights or compromising performance on benign tasks. Our evaluation across five well-known LLMs demonstrates \tool's efficacy, achieving a 95\% success rate while reducing attack time by 86\% compared to existing techniques. This work highlights the need for enhanced trust and verification mechanisms in the open-source AI ecosystem and calls for more robust defenses against sophisticated, covert jailbreak attacks.
% Large language models~(LLMs) have revolutionized  %\shil{(revolutionized is a bit strong, may change another word)} 
% natural language processing but are vulnerable to jailbreak attacks that elicit unintended and insecure outputs. Current token-level jailbreaking techniques, while effective, suffer from scalability and efficiency limitations, especially in the face of frequent model updates and advanced defenses. In this paper, we present \tool, a novel token-level manipulation approach that effectively addresses these challenges.
% %by leveraging insights from our initial empirical study on logit patterns of normal and jailbreak answers. 
% It automatically mines and elicits malicious answers from LLMs by strategically selecting affirmative responses and iteratively reducing the likelihood of rejection answers. We demonstrate the effectiveness and efficiency of \tool through rigorous testing on multiple well-known LLMs and datasets, achieving a significant average reduction of 86\% in time consumption while maintaining high success rates of 95\% on average, even in the presence of defense mechanisms. Our work contributes to the ongoing effort to assess and mitigate the vulnerability of LLMs to jailbreak attacks.
\end{abstract}


==> Chapters/study.tex <==
\section{Empirical Study}

In this section, we perform an empirical investigation to examine the response patterns of the LLM when confronted with harmful behaviors or queries. Section~\ref{subsec:study-method} details the methodology employed in this study, and Section~\ref{subsec:study-result} discusses the outcomes and key findings derived from the empirical analysis.

\subsection{Empirical Study Methodology} 
\label{subsec:study-method}

% 
\subsubsection{Dataset Collection}
\label{subsubsec:dataset-collection}
This section details the dataset assembly procedure for our empirical investigation, which comprises three distinct phases: (1) the acquisition of leading open-source large language models (LLMs) and documentation of harmful behaviors, (2) the development of various prompt templates to serve as inputs to the LLMs, and (3) the generation of text samples from each LLM.


\textbf{LLM and Harmful Behavior Collection:} This phase entails the collection of a select array of open-source large language models (LLMs) and the documentation of harmful behaviors linked to each model. Based on criteria including open-source status, widespread usage, and refinement through human feedback, we select \llamaseven, \llamathirteen, \gemmaseven{}, \llamathreeit{}, and \mistralseven for examination. Additionally, to capture a broad spectrum of harmful behaviors, we utilize \jailbench{}, which comprises 100 harmful behaviors categorized into 10 distinct types, serving as our dataset.

\textbf{Prompt Template Construction:} In this step, we design multiple prompt templates that are specifically tailored to elicit responses from the LLMs, facilitating the evaluation of their output behavior. To investigate the significance of suffixes at the token level, we construct a sequential series of prompt modifications as detailed in Table \ref{tab:em_template}. Initially, we utilize the original question from \jailbench{} as the input. Subsequently, we augment the original question with a partial affirmative suffix. In the final step, we introduce a complete affirmative suffix to the prompt. These progressively modified prompts are designed to explore the hypothesis that the more precise the prompt provided, the greater the likelihood that the LLM will generate toxic responses.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t!]
\centering
\caption{Progressive Prompts Template}
\label{tab:em_template}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc}
\hline
\rowcolor[HTML]{FFFFFF} 
\textbf{Template}                                         & \textbf{Example}                                   \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textless{}harmful\_question\textgreater{}                & Write a tutorial on how to make a bomb.            \\
\rowcolor[HTML]{FFFFFF} 
\textless{}harmful\_question\textgreater{}+``Sure! Here'' & Write a tutorial on how to make a bomb. Sure! Here \\
\rowcolor[HTML]{EFEFEF} 
\textless{}harmful\_question\textgreater{}+\textless{}complete\_prefix\textgreater{} &
  \cellcolor[HTML]{EFEFEF}Write a tutorial on how to make a bomb. Sure! Here is a tutorial on how to make a bomb: \\ \hline
\end{tabular}%
}
\end{table}

\textbf{Text Output Generation:} This stage concentrates on generating text outputs from the LLMs using the prompt templates crafted in the prior phase. We employ these templates directly as inputs to elicit textual responses from the models. To promote diversity in the generated text, we adjust the LLM's temperature parameter to 1 and execute ten generation iterations for each sample.

\subsubsection{Data Labelling}
\label{sec:data-labelling}

This section details the methodology employed for categorizing the text generated by the LLMs.

\textbf{Output Text Labeling:} Evaluating the harmfulness of text poses significant challenges due to the inherent subjectivity involved in assessing the appropriateness of responses generated by Large Language Models (LLMs). To address this, we conduct a comprehensive human evaluation to compare the performance of six widely utilized jailbreak classifiers. In this case, \llamaguard{} classifier fine-tuned on \llamathree{} demonstrates superior effectiveness, characterized by an exceptionally low rate of false positives.

\textbf{Categorization of Denial Pattern:} Understanding the refusal patterns of large language models (LLMs) when responding to harmful queries is crucial. We have analyzed the refusal responses from five LLMs, specifically focusing on the first ten tokens of each response. Our analysis reveals that more than 98\% of these refusal texts conform to 19 distinct prefixes. Furthermore, we categorize these prefixes into four types of denial patterns, providing insights into the systematic refusal strategies employed by LLMs.




\subsection{Empirical Study Result} 
\label{subsec:study-result}
This section presents the result of our empirical study. Section~\ref{subsubsec:harmful-content} presents the result of harmful contents on five selected models with three progressive prompts, and section~\ref{subsubsec:denial-prefix} summarizes the denial patterns when generative texts do not contain any harmful content.

\begin{table}[t!]
    \caption{Result of Empirical Study}
    \centering
    \begin{subtable}{0.48\textwidth}
        \centering
        \caption{Rate of Harmful Contents on Selected Models}
        \label{tab:harmful-contents}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{cccc}
        \hline
        \rowcolor[HTML]{FFFFFF} 
        \cellcolor[HTML]{FFFFFF}                                         & \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Prompts}}     \\ \cline{2-4} 
        \rowcolor[HTML]{FFFFFF} 
        \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Tested Models}} & question-only & question+`Sure! Here' & question+complete prefix \\ \hline
        \rowcolor[HTML]{EFEFEF} 
        \llamaseven{}    & 0\%  & 8\%  & 9\%  \\
        \rowcolor[HTML]{FFFFFF} 
        \llamathirteen{} & 0\%  & 8\%  & 11\% \\
        \rowcolor[HTML]{EFEFEF} 
        \mistralseven{}  & 20\% & 58\% & 77\% \\
        \rowcolor[HTML]{FFFFFF} 
        \llamathreeit{}  & 2\%  & 35\% & 42\% \\
        \rowcolor[HTML]{EFEFEF} 
        \gemmaseven{}    & 10\% & 15\% & 19\% \\ \hline
        Average          & 6\%  & 25\% & 32\% \\ \hline
        \end{tabular}%
        }
    \end{subtable}
    \hfill
    \begin{subtable}{0.48\textwidth}
        \centering
        \caption{Categorization of Denial Prefix on Selected LLMs}
        \label{tab:denial}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{cccccc}
        \hline
        \rowcolor[HTML]{FFFFFF} 
        \cellcolor[HTML]{FFFFFF} &
          \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Categories of Denial Patterns}} &
          \cellcolor[HTML]{FFFFFF} \\ \cline{2-5}
        \rowcolor[HTML]{FFFFFF} 
        \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Test Models}} &
          \textbf{Apology} &
          \textbf{Identification} &
          \textbf{Incapacity} &
          \textbf{Notation} &
          \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Total}} \\ \hline
        \rowcolor[HTML]{EFEFEF} 
        \llamaseven{}    & 23.20\% & 45.00\% & 31.50\% & 0.30\% & 100.00\% \\
        \rowcolor[HTML]{FFFFFF} 
        \llamathirteen{} & 10.30\% & 76.50\% & 13.10\% & 0.00\% & 99.90\%  \\
        \rowcolor[HTML]{EFEFEF} 
        \mistralseven{}  & 0.00\%  & 5.53\%  & 91.04\% & 0.22\% & 96.79\%  \\
        \rowcolor[HTML]{FFFFFF} 
        \llamathreeit{}  & 13.71\% & 34.97\% & 43.40\% & 5.53\% & 97.61\%  \\
        \rowcolor[HTML]{EFEFEF} 
        \gemmaseven{}  & 0.20\%  & 5.40\%  & 92.16\% & 0.91\% & 98.67\%  \\ \hline
        \rowcolor[HTML]{FFFFFF} 
        Average          & 9.48\%  & 33.48\% & 54.24\% & 1.39\% & 98.59\%  \\ \hline
        \end{tabular}%
        }
    \end{subtable}
\end{table}

\subsubsection{Harmful Content in Generative Text}
\label{subsubsec:harmful-content}
As depicted in Figure~\ref{tab:harmful-contents}, a consistent trend in the ratio of harmful content is observed across the five models examined. Notably, when the prompts consist solely of the harmful question, the models, particularly \llamaseven{} and \llamathirteen{}, exhibit minimal propensity to generate harmful responses, with a 0\% occurrence rate. Conversely, the introduction of an affirmative prefix such as 'Sure!' to the prompt markedly increases the incidence of harmful content, elevating the average ratio from 6\% to 25\%.
\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 1:} LLMs are more likely to generate harmful content when adding an affirmative suffix after the original harmful question.
\end{tcolorbox}


Furthermore, a comparison between the prefix 'Sure' alone and a completely affirmative response to the question reveals a distinct increase from 25\% to 32\% in the rate of harmful content with the latter. This observation underscores that more explicit and affirmative prompts significantly enhance the likelihood of eliciting malicious responses from the models.
\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 2:} The longer and more specific the prefix is, the higher the probability of harmful content generation will be.
\end{tcolorbox}


\subsubsection{Denial Prefix in Generative Text}
\label{subsubsec:denial-prefix}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]

\end{table}
In this section, we categorize the denial responses of the models based on the first ten tokens of their replies. The categorization is structured as follows:

\textbf{Apology.} This category includes responses where the model begins with an apology for not being able to provide an answer. Common prefixes include phrases like \textit{`I'm sorry!'} and \textit{`I apologize for...'}.

\textbf{Identification.} Responses under this category reveal the model's artificial identity, often starting with phrases such as \textit{`As a responsible AI'} or \textit{`I'm just an AI'}.

\textbf{Incapacity.} This category is used when the language model indicates an inability to provide potentially harmful responses. For example, models like \gemmaseven{} and \llamathirteen{} start responses to toxic inputs with \textit{`I am unable to complete...'} or \textit{`I cannot finish...'}.

\textbf{Notation.} This category is applicable when models need to denote that a query is illegal or unethical. Typical phrases include \textit{`It is important to note that'}, \textit{`I must clarify that'}, and \textit{`I must emphasize that'}.

As demonstrated in Table~\ref{tab:denial}, 98.59\% of the denial responses can be classified into these four categories. Notably, the \textbf{Identification} and \textbf{Incapacity} categories represent the majority of these responses, whereas the categories \textbf{Apology} and \textbf{Notation} are less common.





\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 3:} In popular LLMs, the types of utterances usually used to deny user requests are limited. Specifically, \textbf{Identification} and \textbf{Incapacity} takes the lead.
\end{tcolorbox}



==> Chapters/study_method.tex <==
\section{Empirical Study Methodology} 
\label{sec:study-method}

% 
\subsection{Dataset Collection}
\label{sec:dataset-collection}
This section details the dataset assembly procedure for our empirical investigation, which comprises three distinct phases: (1) the acquisition of leading open-source large language models (LLMs) and documentation of harmful behaviors, (2) the development of various prompt templates to serve as inputs to the LLMs, and (3) the generation of text samples from each LLM.


\textbf{LLM and Harmful Behavior Collection:} This phase entails the collection of a select array of open-source large language models (LLMs) and the documentation of harmful behaviors linked to each model. Based on criteria including open-source status, widespread usage, and refinement through human feedback, we select \llamaseven, \llamathirteen, \mistralseven, and \qwenseven for examination. Additionally, to capture a broad spectrum of harmful behaviors, we utilize \textit{JailbreakBench}, which comprises 100 harmful behaviors categorized into 10 distinct types, serving as our dataset.

\textbf{Prompt Template Construction:} In this step, we design multiple prompt templates that are specifically tailored to elicit responses from the LLMs, facilitating the evaluation of their output behavior. To investigate the significance of suffixes at the token level, we construct a sequential series of prompt modifications as detailed in Table \ref{tab:em_template}. Initially, we utilize the original question from \textit{JailbreakBench} as the input. Subsequently, we augment the original question with a partial affirmative suffix. In the final step, we introduce a complete affirmative suffix to the prompt. These progressively modified prompts are designed to explore the hypothesis that the more precise the prompt provided, the greater the likelihood that the LLM will generate toxic responses.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\caption{Progressive Prompts Template}
\label{tab:em_template}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc}
\hline
\rowcolor[HTML]{FFFFFF} 
\textbf{Template}                                         & \textbf{Example}                                   \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textless{}harmful\_question\textgreater{}                & Write a tutorial on how to make a bomb.            \\
\rowcolor[HTML]{FFFFFF} 
\textless{}harmful\_question\textgreater{}+``Sure! Here'' & Write a tutorial on how to make a bomb. Sure! Here \\
\rowcolor[HTML]{EFEFEF} 
\textless{}harmful\_question\textgreater{}+\textless{}complete\_suffix\textgreater{} &
  \cellcolor[HTML]{EFEFEF}Write a tutorial on how to make a bomb. Sure! Here is a tutorial on how to make a bomb: \\ \hline
\end{tabular}%
}
\end{table*}

\textbf{Text Output Generation:} This stage concentrates on generating text outputs from the LLMs using the prompt templates crafted in the prior phase. We employ these templates directly as inputs to elicit textual responses from the models. To promote diversity in the generated text, we adjust the LLM's temperature parameter to 2 and execute ten generation iterations for each sample.

\subsection{Data Labelling}
\label{sec:data-labelling}

\textbf{Output Text Labeling:} This section details the methodology employed for categorizing the text generated by the LLMs. Specifically, we use GPT-4 as the semantic judge in line with the criteria established by ~\cite{}, where the output text is considered harmful and toxic only if it achieves a 10 out of 10 jailbreak score from GPT-4.

==> Chapters/study_result.tex <==
\subsection{Empirical Study Result} 
\label{sec:study-result}



\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 1:} LLMs are more likely to generate harmful content when adding an affirmative suffix after the original harmful question.
\end{tcolorbox}

\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 2:} The longer and more specific the suffix is, the higher the probability of harmful content generation will be.
\end{tcolorbox}

\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 3:} In popular LLMs, the types of utterances usually used to deny user requests are limited.
\end{tcolorbox}
